Semi-Supervised Hierarchical Drug Embedding in Hyperbolic Space

Learning accurate drug representation is essential for tasks such as computational drug repositioning and prediction of drug side-effects. A drug hierarchy is a valuable source that encodes human knowledge of drug relations in a tree-like structure where drugs that act on the same organs, treat the same disease, or bind to the same biological target are grouped together. However, its utility in learning drug representations has not yet been explored, and currently described drug representations cannot place novel molecules in a drug hierarchy. Here, we develop a semi-supervised drug embedding that incorporates two sources of information: (1) underlying chemical grammar that is inferred from molecular structures of drugs and drug-like molecules (unsupervised), and (2) hierarchical relations that are encoded in an expert-crafted hierarchy of approved drugs (supervised). We use the Variational Auto-Encoder (VAE) framework to encode the chemical structures of molecules and use the knowledge-based drug-drug similarity to induce the clustering of drugs in hyperbolic space. The hyperbolic space is amenable for encoding hierarchical concepts. Both quantitative and qualitative results support that the learned drug embedding can accurately reproduce the chemical structure and induce the hierarchical relations among drugs. Furthermore, our approach can infer the pharmacological properties of novel molecules by retrieving similar drugs from the embedding space. We demonstrate that the learned drug embedding can be used to find new uses for existing drugs and to discover side-effects. We show that it significantly outperforms baselines in both tasks.

==> sections/setup_v2.tex <==
\section{Problem Setup}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/KDD_schematic_diagram_v5.png}
    %\caption{Schematic diagram of the proposed drug embedding framework. Our approach can be viewed as a semi-supervised learning which combines a small amount of FDA-approved drugs ($X_\mathrm{FDA}$) classified in the ATC ($\mathcal{T}$) and a large amount of unnamed drug-like molecules ($X_\mathrm{ZINC}$) drawn from the ZINC database. We use VAE to encode molecules into a hyperbolic space $\mathbb{H}^n$. We inject the ATC hierarchy in the embedding space by preserving local similarity rankings of drugs. Notations: $\bm{x}$, $\bm{z}$, $\hat{\bm{x}}$ denote a SMILES string, its embedding and its reconstruction; $q_\phi(\bm{z}|\bm{x}), p_\theta(\bm{x}|\bm{z})$ denote encoder network and decoder network respectively; $\mathcal{L}_\mathrm{ELBO}(\bm{x};\phi,\theta)$, $\mathcal{L}_\mathrm{SLR}(\bm{x},\mathcal{T};\phi)$ denote the objective functions of VAE and local similarity rankings.}
    
    \caption{Schematic diagram of the proposed drug embedding method. Our semi-supervised learning approach integrates the chemical structures of a small number of FDA-approved drug molecules ($X_\mathrm{FDA}$) and a larger number of drug-like molecules ($X_\mathrm{ZINC}$) drawn from the ZINC database. We use VAE to encode molecules in hyperbolic space $\mathbb{H}^n$, and enforce the ATC drug hierarchy by preserving local similarity rankings of drugs. The symbols $\bm{x}$, $\bm{z}$, $\hat{\bm{x}}$ denote a molecule represented by its SMILES string, its embedding and its reconstruction; $q_\phi(\bm{z}|\bm{x}), p_\theta(\bm{x}|\bm{z})$ denote the encoder network and the decoder network respectively; $\mathcal{L}_\mathrm{ELBO}(\bm{x};\phi,\theta)$, $\mathcal{L}_\mathrm{SLR}(\bm{x},\mathcal{T};\phi)$ denote the objective functions for the VAE and the local similarity rankings.}
    \label{fig:1}
\end{figure*}



\noindent We develop a drug embedding that integrates the chemical structures of drug-like molecules with a drug taxonomy such that the similarity between pairs of drugs is informed both by the structure and groupings in the taxonomy. To learn the underlying grammar of chemical structures, we leverage a data set of drugs (about 1.3K) that are approved by the Food and Drug Administration (FDA) and a larger data set of drug-like molecules (about 250K) and use the simplified molecular-input line-entry system (SMILES)~\cite{weininger1988smiles} structure representation. We obtain additional drug similarity relationships from the Anatomical Therapeutic Chemical (ATC) drug taxonomy that provides a tree-like hierarchy of drug groupings. We use the hyperbolic space for the embedding since it is amenable for learning continuous concept hierarchies~\cite{nickel2017poincare, nickel2018learning,mathieu2019continuous,de2018representation, monath2019gradient, nagano2019wrapped}.

We formulate the learning of the drug embedding as a Variational Auto-Encoder where the codes ($\bm{z}$) reside in hyperbolic space. More specifically, we adopt a variant that replaces the prior normal distribution in the VAE with the so-called wrapped normal distribution in the Lorentz model of hyperbolic space to leverage its numerical stability~\cite{nickel2018learning, nagano2019wrapped}. To integrate the hierarchical relationships from the drug taxonomy, we use a loss function that enforces the pairwise hyperbolic distance between drugs to be consistent with pairwise shortest path lengths in the ATC tree.

%In summary, we develop a drug embedding in hyperbolic space (see Figure~\ref{fig:1}) that consists of two learning tasks: (1) applying a hyperbolic VAE to extract the underlying grammar of structures of drug and drug-like molecules; and (2) enforcing the ATC hierarchy in the embedding space by preserving local similarity orderings of drugs.



